CIC: Contrastive Intrinsic Control for Unsupervised Skill Discovery

We introduce Contrastive Intrinsic Control (CIC), an algorithm for unsupervised skill discovery that maximizes the mutual information between state-transitions and latent skill vectors. CIC utilizes contrastive learning between state-transitions and skills to learn behavior embeddings and maximizes the entropy of these embeddings as an intrinsic reward to encourage behavioral diversity. We evaluate our algorithm on the Unsupervised Reinforcement Learning Benchmark, which consists of a long reward-free pre-training phase followed by a short adaptation phase to downstream tasks with extrinsic rewards. CIC substantially improves over prior methods in terms of adaptation efficiency, outperforming prior unsupervised skill discovery methods by 1.79x and the next leading overall exploration algorithm by 1.18x.

==> sections/related.tex <==
\section{Related Work}

{\bf Supervised Reinforcement Learning:} To date, most of RL research has focused on supervised RL where training is supervised with an extrinsic reward function. Supervised RL has seen many breakthroughs over the last five years~\citep{mnih2015human, alphago, alphastar, alphazero, berner2019dota,andrychowicz2020learning, schulman2015high, ppo}. The field has also produced several stable RL optimization algorithms that have helped accelerated research~\cite{sac,hessel18rainbow,lillicrap15ddpg,ppo}.

{\bf Unsupervised Reinforcement Learning:} The sub-field of unsupervised RL consists of two primary research areas - {\it unsupervised behavioral learning} and {\it unsupervised representation learning}~\citep{srinivas_abbeel_2021_icml_tutorial}. Unsupervised behavioral learning consists of learning behaviors and exploring the environment without extrinsic rewards. Unsupervised representation learning consists of learning representations without supervision from high-dimensional data such as pixel observations. We evaluate our method on the recently introduced Unsupervised RL Benchmark (URLB)~\citep{laskin_yarats_2021_urlb}, and focus solely on the behavioral aspect of unsupervised RL in order to isolate the core issue preventing prior unsupervised skill discovery methods from exploring effectively on URLB. 



{\bf Unsupervised Behavioral Learning:} The aim of unsupervised behavioral learning is to produce diverse behaviors that explore the environment without interacting with an extrinsic reward. Often referred to as intrinsic motivation~\citep{oudeyer2007intrinsic}, this is typically achieved by defining an intrinsic reward through a self-supervised task. Most behavioral learning algorithms fall into three categories -- knowledge-based~\citep{pathak2017curiosity,Pathak19disagreement, burda2018exploration, burda2018largescale} where the agent maximizes the error or uncertainty of some predictive model, data-based~\citep{campos2021beyond,liu2021unsupervised,  liu21aps,mutti2020policy,seo21re3,yarats21protorl} where the agent maximizes data diversity, and competence-based~\cite{EysenbachGIL19diayn,hansen20visr,liu21aps,SharmaGLKH20dads} where the agent maximizes the mutual information between observable variables and a latent skill vector. We discuss the differences between \name and the most closely related competence-based exploration algorithms in Appendix~\ref{appendix:prior_skills}.

{\bf Unsupervised Representation Learning:} Much progress in unsupervised representation learning for RL has been spurred by unsupervised learning in computer vision~\citep{chen2020simclr,he2020moco,henaff2019cpcv2, kingma2013auto} and language~\citep{brown2020language,devlin2018bert,radford2019language}. In RL, the most common approach for representation learning has been by adding it as an auxiliary loss in the supervised RL setting~\citep{jaderberg17unreal}. More recently, a number of works have investiagted representaton learning with autoencoders~\citep{yarats2019improving, hafner2018learning,hafner2019dream}, siamese networks~\citep{schwarzer2021dataefficient, schwarzer2021pretraining, laskin2020curl,stooke2020decoupling,yarats21protorl}, and data augmentation~\citep{laskin2020reinforcement,yarats2021drqv2,yarats2021image}. 
